Private Order Flows and Builder Bidding Dynamics: The Road to Monopoly in Ethereum's Block Building Market

Ethereum, as a representative of Web3, adopts a novel framework called Proposer Builder Separation (PBS) to prevent the centralization of block profits in the hands of institutional Ethereum stakers. Introducing builders to generate blocks based on public transactions, PBS aims to ensure that block profits are distributed among all stakers. Through the auction among builders, only one will win the block in each slot. Ideally, the equilibrium strategy of builders under public information would lead them to bid all block profits. However, builders are now capable of extracting profits from private order flows. In this paper, we explore the effect of PBS with private order flows. Specifically, we propose the asymmetry auction model of MEV-Boost auction. Moreover, we conduct empirical study on Ethereum blocks from January 2023 to May 2024. Our analysis indicates that private order flows contribute to 54.59% of the block value, indicating that different builders will build blocks with different valuations. Interestingly, we find that builders with more private order flows (i.e., higher block valuations) are more likely to win the block, while retain larger proportion of profits. In return, such builders will further attract more private order flows, resulting in a monopolistic market gradually. Our findings reveal that PBS in current stage is unable to balance the profit distribution, which just transits the centralization of block profits from institutional stakers to the monopolistic builder.

==> sections/3-Datasets.tex <==
\section{Datasets}
\subsection{Data Collections}

\subsubsection{Builder MEV-Boost Auction}

During a single time slot, builders consistently employ optimization algorithms to package blocks and transmit them to the relays. Consequently, we undertake the aggregation of the bidding processes occurring within the builder's off-chain layer by interfacing with diverse relay APIs. Specifically, we acquire all bidding processes by utilizing the `builder blocks received' endpoint of these APIs. 


During the slot interval, the relay arranges the received blocks based on priority fees for proposers and submits the most profitable ones. The `proposer payload delivered' endpoint of the relay API reveals all the blocks chosen by proposers for inclusion. Network latency introduces timing uncertainty in relay submissions, potentially resulting in missed opportunities with the most profitable blocks.  

\subsubsection{On-chain Data.~}
We deployed a Geth node and a Prysm node to sync the block and the transaction information.

\subsubsection{Public Mempool Transactions.~}
Using Flashbots Mempool Dumpster~\cite{flashbots-mempool}, we collected public mempool data. This data set is updated on a daily basis and provides data including the time when a transaction was first detected, the time when the transaction was included in the block, the cost of the transaction, and more.

